Embedded Finite Models Beyond Restricted Quantifier Collapse

We revisit evaluation of logical formulas that allow both uninterpreted relations, constrained to be finite, as well as an interpreted vocabulary over an infinite domain. This formalism was denoted embedded finite model theory in the past. It is clear that the expressiveness and evaluating complexity of formulas of this type depends heavily on the infinite structure. If we embed in a wild structure like the integers with additive and multiplicative arithmetic, logic is extremely expressive and formulas are impossible to evaluate. On the other hand, for some well-known decidable structures, the expressiveness and evaluating complexity are similar to the situation without the additional infrastructure. The latter phenomenon was formalized via the notion of ``Restricted Quantifier Collapse'': adding quantification over the infinite structure does not add expressiveness. Beyond these two extremes little was known. In this work we show that the possibilities for expressiveness and complexity are much wider. We show that we can get almost any possible complexity of evaluation while staying within a decidable structure. We also show that in some decidable structures, there is a disconnect between expressiveness of the logic and complexity, in that we cannot eliminate quantification over the structure, but this is not due to an ability to embed complex relational computation in the logic. We show failure of collapse for the theory of finite fields and the related theory of pseudo-finite fields, which will involve coding computation in the logic. As a by-product of this, we establish new lower-bounds for the complexity of decision procedures for several decidable theories of fields, including the theory of finite fields. In the process of investigating this landscape, we investigate several weakenings of collapse.

==> app_bezout.tex <==
\section{Proof of Theorem \ref{thm:bezout}: solution  bounds used in the lower bounds for pseudo-finite fields}
Recall the statement:

\medskip

There is an elementary function $F$ such that in any pseudo-finite field
if $\theta(\vec u, \vec v)$ is a basic formula
and for a given $\vec u$ the set $\theta_{\vec u}$ of $\vec v$ such that $\theta(\vec u, \vec v)$ holds is finite,
then $|\theta_{\vec u}|$ has size bounded by $F(size(\theta))$. Here size of $\theta$ takes into account the degrees of the polynomials
in addition to the number of terms.


\medskip

Recall that a basic formula is an existential quantification of a conjunction of polynomial equalities,
with only one existential quantifier.
The result can be restated in terms of \emph{finite fields}:
if we we have a basic formula $\theta$ where the size of solutions is bounded as we range over all finite fields 
and parameters $\vec u$, then the size must be bounded by an elementary function.


We first argue for a similar statement that removes the existential quantification:


\begin{theorem} \label{thm:bezoutatomic}
There is an elementary function $F$ such that in any pseudo-finite field 
if $\theta(\vec u, \vec v)$ is a conjunction of polynomial equalities
and for a given $\vec u$ the set $\theta_{\vec u}$ of $\vec v$ such that $\theta(\vec u, \vec v)$ holds is finite,
then $|\theta_{\vec u}$ has size $F(size(\theta))$. Here size takes into the degrees of the polynomials
in addition to the number of terms.
\end{theorem}


We need some auxiliary definitions. 
The theory of  Algebraically Closed Fields with an Automorphism 
(ACFA) is in the language of an algebraically closed field $F$ with a distinguished automorphism $\sigma$ satisfying
certain axioms, one of which is that it is a \emph{difference-closed difference field}.

The axioms will not concern us. The only thing that is important to us is:

\begin{proposition} \label{prop:acfa}
Every pseudo-finite field is the fixed field of $(K, \sigma)$ that is a model of ACFA.
\end{proposition}

See, for example, \cite{garcia}, comments after Proposition 4.3.6.
The proposition above allows us to reduce reasoning about polynomial equalities within a pseudo-finite
field, which is not algebraically closed, to reasoning within the fixed field of an algebraically
closed field with a suitable automorphism. We can thus think of our solution set as the conjunction
of the polynomial equalities along with the ``difference equation'' $\sigma(x)=x$''.



An \emph{affine variety} over a field $K$ is a set of elements $K$ defined by 
polynomial equations with coefficients in the field.  So we are interested in the intersection
of an affine variety with a simple difference equation.



We now state Proposition 2.2.1 of \cite{emm}:

\begin{proposition} \label{prop:emm} Let $(K;  \sigma)$ be 
a difference-closed difference field; and let $S$ be a
 subvariety of $\mathcal{P}^l$
 defined over $K$. Let $Z$ be the Zariski closure of 

\[
\{x \in \mathcal{P}:(x,  \sigma(x) \ldots \sigma^{l-1}(x)) \in S\}
\]
Then $deg(Z) \leq deg(S)^{dim(S)}$. 
In particular; $Z$ has at most $deg(S)^{dim(S)}$
irreducible components.
\end{proposition}



We explain the route from Proposition \ref{prop:emm} to Theorem \ref{thm:bezoutatomic}, introducing
the relevant terminology from Proposition \ref{prop:emm} as needed.
Proposition \ref{prop:emm} is stated for a subvariety of a projective variety: this is
$\mathcal{P}^l$. Again, we will not
need the definition of projective varieties, but note that an  affine variety 
can be embedded
in a projective variety in a way that preserves number of solutions (by adding additional variables and
equations). Thus the same proposition also holds for an affine variety $S$ sitting within
another affine variety.

Proposition \ref{prop:emm} also refers to the Zariski closure, degree, and dimension.  But
if a variety is finite, its Zariski closure is just itself, the   degree is the number of points, and
the dimension is upper bounded by the number of variables in the defining polynomials.
With that in mind, let us explain the derivation of Theorem \ref{thm:bezout} from
Proposition \ref{prop:emm}.

In Proposition \ref{prop:emm} we  apply Proposition \ref{prop:acfa},
fixing an algebraically closed field $K$ and an automorphism  $\sigma$ with $(K, \sigma) \models ACFA$,
 such that our pseudo-finite field is the  fixed field
of $K$ under $\sigma$.
Thus the set we are interested in is 
\[
\{x | \{(x, \sigma(x) \ldots \sigma^{l-1}(x)) \in S\}
\]
 where $S$
is the subvariety of the product of our  variety with itself, adding
the additional equation saying that the components are all equal.
Proposition \ref{prop:emm} tells us that the degree of this subvariety is  bounded by
 $deg(S)^{dim(S)}$. By the comments above about degree and dimension for finite set,
this is an exponential in the size, so we are done.


Theorem \ref{thm:bezoutatomic}  deals only  with a formula $\psi(\vec u, \vec x, \vec y)$
which is a conjunction of  polynomial equalities.
While
Theorem \ref{thm:bezout} is the projection of such a conjunction: of the form
 $\exists  y ~ \psi(\vec u, \vec x, y)$.
 Our hypothesis is that this projection has finitely many solutions, which does not allow
us to conclude that $\psi$ has only finitely many.
There
are several ways to handle this.

First, we can note that when $\vec u, \vec x$ are non-zero, there can only be finitely many
$y$ such that  $\psi(\vec u, \vec x, y)$ holds.  We can think of the $\vec u, \vec x$ as 
coefficients
on a polynomial in one variable.
Thus we can disjoin over guesses
as to which $\vec u, \vec x$  are non-zero in a solution. Each such disjunct can be captured by
polynomial equalities along with a negated equality, with the latter asserting that certain
 but inequalities  $\tau(\vec w) \neq 0$ can be converted to equalities by adding
an  existential $\exists u  ~ \tau(\vec x) \cdot u-1=0$. This may seem circular, since we have added
back in an existential. But there is a unique $(u,\vec w)$ for each $\vec w$ satisfying $\tau(\vec w) \neq 0$,
these existentials do not blow up the number of solutions.

Another approach is to use Proposition \ref{prop:emm}, but relies on a bit more algebraic geometry.

Let  $X= \{\vec x, \vec u, y | \psi(\vec x, \vec u, y)\}$. Let $cl(U)$ for any $U$ be the Zariski
Closure,   and let
$NCom(X)$ be the number of irreducible components of the Zariski closure of $X$.
i.e. the smallest number $n$ such that $X$ can be covered by $n$ irreducible varieties $V$ with 
$X \meet V$ dense in $V$.    
The argument from Proposition \ref{prop:emm} allows us to obtain an elementary bound on
$NCom(X)$ in terms of the size of $\phi$ -- without assuming finiteness of $X$.

Let us assume $\pi(X)$ is finite.
We have $\pi(cl(X)) \subset cl(\pi(X))$ always, and when $\pi(X)$ is finite $cl(\pi(X) = \pi(X)$.
Thus  $\pi(cl(X))$ is also finite.
For each irreducible component $C$ in $Cl(X)$,
we have $\pi(C)$ is finite, so it must be a point.  Hence $|\pi(X) | \leq NumCom(X)$, and
we get an elementary bound on $|\pi(X)|$.





==> app_higher.tex <==
\section{Proof of Proposition \ref{prop:spectrum}: separating pure spectra }

Recall the statement:

\medskip

For any $k$, there is a set $J_k$ of integers that is the spectrum of a $k+2$-order logic
sentence in pure equality but not the spectrum of the sentence of any  $k$-order logic sentence over pure equality

\medskip

Note that for formulas with only equality, there is a one-to-one correspondence between models of the formula and integers, where the correspondence
maps a model to its size. Thus it is enough to separate the expressiveness of $k+2$ order logic from that of $k$ order logic, over a unary signature.
We have

This follows from results  in \cite{mostowskisemantics,leszek}, stating that a truth definition for a $k$ order logic  sentence can always
be expressed as $k+2$ order logic sentence. This holds for any fixed signature, hence also for a fixed signature.

Note that \cite{hellahigherorder,hullsuhigherorder} claim separation results for expressibility in higher-order logic,  following
from complexity characterizations of the definable sets in the logic: in \cite{hellahigherorder} the characterization is via non-deterministic iterated
exponential time with an oracle for a class in the polynomial hierarchy. Similar characterizations are provided in \cite{leszek}.
In \cite{hellahigherorder}, the argument that is sketched for separation does not apply to a signature with only equality
%Further the main separation theorem (Corollary 11 in \cite{hellahigherorder}) is not proven. 
In \cite{hullsuhigherorder} the  argument for separation relies on unpublished results in a Phd thesis \cite{thesisspectrum}, so it is difficult to say the signatures to which it applies.
But it seems likely that the separation result does not apply to the case of a trivial signature.  


==> app_separate.tex <==
\section{Making the separating families Simple}

Recall that in the body we had theories that were $k+2$-RQC but not $k$-RQC.
We claimed that  we could modify to enforce that the examples are \emph{simple theories}, thus
disproving the notion that simplicity is enough to gain $k$-RQC or even $\omega$-RQC.
In fact we can obtain theories to have 
``SU-rank $1$''.
Simple theories have many equivalent definitions, one of which is that they ``do not have the tree property'': there is no partitioned formula $\phi(\vec x; \vec y)$ and an infinite tree of instantiations
$\phi(\vec x, \vec a)$ so that: the formulas along each branch are consistent, but the formulas
associated to children of a given node are inconsistent.
For our purposes, the full definitions of simple and SU-rank are not needed, and since a tutorial
on simplicity is outside the scope of this paper, we omit these definitions.
For alternative definitions of simplicity, forking, and SU-rank, and for
the proof that SU-rank $1$ implies simplicity, we
refer to \cite{wagnersimple}.  We will only need to know that a certain property that we can define
directly -- no non-trivial dividing -- suffices to give simplicity.
Our proof below can easily be converted to a direct argument that
the theories do not have the tree property.


%given P we want to test that |P| is in: we test whether 
To get this property of a Fra\"isse limit, we modify the signature used in the body
by adding  a $4$-ary predicate $F(x,y, w, z)$.
Given a set of integers $J$ we now consider the set of finite structures for $R,Z,F$
such that $R(x,y,z)$ implies $x,y, z$ are all distinct,
and for no $a$ in the domain do we have that
$B(n)$ embeds as an induced substructure of $R_a$ 
\emph{and}   for all vertices $b,c,d$ of $R_a$, $F(a, b,c,d)$ holds.

The class of structures above has the Amalgamation Property, Hereditary Property, and the Joint
Embedding Property, and thus there is a Fra\"isse limit whose finite substructures are the structures
in the class.
We can still test whether $|P|$ is in $J$ by forming a structure whose $R$ structure
is $B(|P|)$ and testing when there there is an $a$  with $R_a$ embedding the
structure and $F$ connecting $a$ to every pair in the structure.

We can still reduce $L_P$ formulas to testing whether $|P|$ is in $J$, by guessing
not only the graphs $G_1, G_2, G_3$ and also the $F$ structure.

What remains is now to show that this modification ensures that the limit structure is simple.
We will argue first that the class has a stronger amalgamation property than the amalgamation property
mentioned above.
The property is \emph{$3$-amalgamation}, defined as follows:

\medskip

Suppose we have $3$ structures $A_1, A_2, A_3$ in the class extending the same substructure $A$, and suppose
for each pair $A_i, A_j$ there is a structure $A_{ij}$ in the class such that we can jointly
 embed $A_i, A_j$ into $A_{ij}$ while identifying $A$: that is, we can amalgamate each pair.
Then there is $A_{1,2,3}$ in the class and  embeddings of $A_1, A_2, A_3$ into $A_{1,2,3}$ that preserve $A$.

\medskip

To get some intuition for the property, note that the class of all graphs has $3$-amalgamation,
but the class of triangle-free graphs has amalgamation but does \emph{not} have $3$-amalgamation:
we consider $A_1$, $A_2$, $A_3$ each consist of a single edge of a triangle. Each pair of structures
can be amalgamated, but the triple cannot be: one can consider
this as a canonical example of how $3$-amalgamation can fail.
Thus the class of triangle-free graphs has a  Fra\"isse limit -- the ``universal triangle-free graph'' --
but the theory of this structure is not simple.

To prove $3$-amalgamation,  it suffices to consider three models $B, C, D$ consisting
of a common overlapping domain $A=\{a_1,\ldots,a_n\}$ along
with one additional  element in each, denoted  $b,c,d$ respectively.
 To amalgamate, we  take a structure
$E$ that is the disjoint union. For $a \in A$ we cannot have $R_a$ violate the property
above on a graph $R_a$ with $R_a$ not containing all $3$ of $b,c,d$,
 by the assumption of pairwise compatibility on the models $B,C,D$.
We cannot have $R_a$ violate the property on a graph that contains all of $b,c,d$ since
the relation $F$ will not hold.

A \emph{non-trivial dividing} consists of a  formula
 $\phi(\vec x; \vec y)$,  set $A$,  and a sequence
$\vec a_1 \ldots$ indiscernible over $A$ such that for each $i$, $\phi(\vec x, \vec a_i)$ is consistent but
the whole collection $\phi(\vec x, \vec a_i)$ is inconsistent. If there is no non-trivial dividing, then the
SU-rank of the theory is $1$, and in particular the theory is simple.

We claim that $3$-amalgamation implies that there can be no non-trivial dividing.
This is surely known (e.g. implicit in \cite{conantamalg}), but we give an argument for completeness.
Consider the three structures
$\vec x  \vec a_1 A$,  $\vec a_1, \vec a_2 A$, $\vec x, \vec a_2, A$ where $\phi(\vec x, \vec a_1)$ holds in the first and $\phi(\vec x, \vec a_2)$ holds
in the third. The fact that $\phi(\vec x, \vec a_i)$ is consistent implies that each pair can be amalgamated. hence there is
a structure amalgamating all $3$.  Iterating this argument inductively gives the desired result.












